DataFlow-Harness: A Grounded Code-Agent Platform for Constructing Editable LLM Data Pipelines

Large language models (LLMs) are increasingly used to automate data-processing workflows, yet coding agents typically produce scripts that are not automatically materialized as persistent, editable platform artifacts. We call this disconnect the \textit{NL2Pipeline gap}. To bridge it, we introduce \textsc{DataFlow-Harness}, a platform that guides an LLM agent to construct platform-native directed acyclic graphs (DAGs) through typed, incremental mutations rather than free-form scripts. The platform combines \textsc{DataFlow-Skills} for procedural guidance, a Model Context Protocol (MCP) layer that exposes the live operator registry and current pipeline state, and \textsc{DataFlow-WebUI}, which synchronizes conversational authoring with a visual DAG editor. On a 12-task data-engineering benchmark, \textsc{DataFlow-Harness} achieves a 93.3\% observed end-to-end pass rate. Relative to Vanilla Claude Code, it reduces measured monetary cost by 72.5\% and generation latency by 49.9\%; its observed pass rate is within 0.9 percentage points of the Context-Aware Claude Code baseline while its cost is 42.8\% lower. Per-task analysis indicates that Skills are most useful when construction depends on implicit procedural knowledge. These results show that live platform grounding can produce persistent, editable workflow artifacts with an observed reliability close to script-generation baselines and with lower measured construction cost and latency.

==> tables/agenticrag.tex <==
\begin{table}
\centering
\small
\caption{AgenticRAG Pipeline: Performance comparison between synthetic datasets and existing human-constructed datasets. All values are Exact Match (\%). ``OOD-Avg'' excludes the in-domain test set of each training dataset. ``DF-OOD (matched)'' provides the OOD score of DF-AgenticRAG under the *same* in-domain exclusion, ensuring fair comparison.}
\label{tab:agenticrag}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Training Data} & \textbf{HotpotQA} & \textbf{2Wiki} & \textbf{Musique} & \textbf{Bamboogle} & \textbf{Avg} & \textbf{OOD-Avg} & \textbf{DF-OOD (matched)} \\
\midrule
Qwen-2.5-7B-Instruct & 25.0 & 25.8 & 9.9 & 27.2 & 22.0 & -- & -- \\
\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               HotpotQA group
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{Trained on HotpotQA (in-domain = HotpotQA)}}} \\
\midrule

HotpotQA-10k (1 epoch) & 40.2 & 41.9 & 16.7 & 42.4 & 35.3 & 33.7 & \textbf{33.8} \\
HotpotQA-10k (2 epochs) & 43.4 & 44.9 & 18.9 & 41.6 & 37.2 & 35.1 & \textbf{35.9} \\
HotpotQA-10k (3 epochs) & 45.3 & 48.0 & 20.3 & 40.8 & 38.6 & 36.4 & \textbf{37.4} \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               Musique group
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{Trained on Musique (in-domain = Musique)}}} \\
\midrule

Musique-20k (1 epoch) & 41.1 & 44.7 & 19.2 & 41.6 & 36.6 & 42.4 & \textbf{43.6} \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               2Wiki group
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{Trained on 2Wiki (in-domain = 2Wiki)}}} \\
\midrule

2Wiki-30k (2 epochs) & 41.3 & 55.1 & 17.8 & 42.4 & 39.1 & 33.8 & \textbf{36.4} \\

\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            DF-AgenticRAG raw
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor[rgb]{.867,.922,.969}
\multicolumn{8}{c}{\textit{\textbf{DF-AgenticRAG (raw results, for reference)}}} \\
\midrule

DataFlow-AgenticRAG-10k (1 epoch) & 39.3 & 42.6 & 17.3 & 41.6 & 34.3 & -- & -- \\
DataFlow-AgenticRAG-10k (2 epochs) & 43.1 & 44.6 & 19.9 & 43.2 & 37.7 & -- & -- \\
DataFlow-AgenticRAG-10k (3 epochs) & 42.6 & 45.5 & 20.2 & 46.4 & 38.7 & -- & -- \\

\bottomrule
\end{tabular}
}
\end{table}


==> tables/code_1.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance comparison of Qwen2.5-7B and Qwen2.5-14B under different SFT dataset settings (all numbers in \%).}
\label{tab:code_1}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{HumanEval} & \textbf{MBPP} & \textbf{BigCodeBench} & \textbf{LiveCodeBench} & \textbf{Avg} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{6}{c}{\textit{\textbf{Trained on Qwen2.5-7B}}} \\
\midrule
Original & 57.9 & 74.9 & 37.5 & 2.5  & 43.2 \\
Code Alpaca & 76.2 & 76.5 & 43.8 & 6.0  & 50.6 \\
Self-OSS-Instruct-SC2-Exec-Filter-50k & 74.4 & 77.0 & 42.7 & 6.1  & 50.1 \\
DataFlow-Code-1K & 75.0 & 75.4 & 46.2 & 21.5 & 54.5 \\
DataFlow-Code-5K & 78.7 & 77.2 & 46.1 & 22.1 & 56.0 \\
DataFlow-Code-10K & 78.7 & 78.3 & 45.9 & 23.0 & \textbf{56.5} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{6}{c}{\textit{\textbf{Trained on Qwen2.5-14B}}} \\
\midrule
Original & 56.7 & 76.7 & 53.4 & 21.2 & 52.0 \\
Code Alpaca & 81.5 & 78.8 & 53.3 & 21.9 & 58.9 \\
Self-OSS-Instruct-SC2-Exec-Filter-50k & 82.0 & 81.0 & 52.2 & 23.6 & 59.7 \\
DataFlow-Code-1K & 77.6 & 82.5 & 53.9 & 27.6 & 60.4 \\
DataFlow-Code-5K & 79.9 & 84.1 & 54.2 & 27.8 & 61.5 \\
DataFlow-Code-10K & 81.1 & 84.5 & 54.1 & 30.0 & \textbf{62.4} \\
\bottomrule
\end{tabular}
}
\end{table}



==> tables/code_2.tex <==
\begin{table}[t]
\centering
\small
\caption{Code Pipeline: Performance comparison of Qwen2.5-7B-Instruct and Qwen2.5-14B-Instruct under different SFT dataset settings (all numbers in \%).}
\label{tab:code_2}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Training Data} & \textbf{BigCodeBench} & \textbf{LiveCodeBench(v6)} & \textbf{CruxEval (Input)} & \textbf{CruxEval (Output)} & \textbf{HumanEval+} & \textbf{Avg} \\
\midrule

\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Trained on Qwen2.5-7B-Instruct}}} \\
\midrule
\textbf{Qwen2.5-7B-Instruct}              & 35.3 & 23.4 & 44.8 & 43.9 & 72.6 & 44.0 \\
\textbf{+ Code Alpaca-1K}        & 33.3 & 18.7 & 45.6 & 46.4 & 66.5 & 42.1 \\
\textbf{+ Self-OSS}              & 31.9 & 21.4 & 46.9 & 45.9 & 70.1 & 43.2 \\
\textbf{+ DataFlow-Code-1K}      & 35.5 & 25.7 & 48.0 & 45.1 & 72.6 & 45.4 \\
\textbf{+ DataFlow-Code-5K}      & 36.2 & \textbf{26.4} & 48.6 & 45.0 & 73.2 & 45.9 \\
\textbf{+ DataFlow-Code-10K}     & \textbf{36.8} & 26.0 & \textbf{48.8} & \textbf{45.4} & \textbf{73.8} & \textbf{46.2} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Trained on Qwen2.5-14B-Instruct}}} \\
\midrule
\textbf{Qwen2.5-14B-Instruct}              & 37.5 & 33.4 & 48.0 & 48.5 & 74.4 & 48.4 \\
\textbf{+ Code Alpaca-1K}        & 37.0 & 28.2 & 50.2 & 49.6 & 71.3 & 47.3 \\
\textbf{+ Self-OSS}              & 36.9 & 22.3 & 52.6 & 50.1 & 68.3 & 46.0 \\
\textbf{+ DataFlow-Code-1K}      & 41.4 & \textbf{33.7} & 51.0 & 50.9 & \textbf{77.3} & 50.9 \\
\textbf{+ DataFlow-Code-5K}      & 41.1 & 33.2 & 52.5 & 50.6 & 76.2 & 50.7 \\
\textbf{+ DataFlow-Code-10K}     & \textbf{41.9} & 33.2 & \textbf{52.9} & \textbf{51.0} & 76.2 & \textbf{51.0} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/dfa_table1.tex <==
\begin{table*}[!h]
\centering
\caption{Agent orchestration performance by evaluation mode and description difficulty.}
\label{tab:agent-orchestration-results-vertical}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\small

\begin{tabular}{lcccc}
\toprule
\textbf{Metric} & \textbf{Easy} & \textbf{Medium} & \textbf{Hard} & \textbf{Overall} \\
\midrule

\multicolumn{5}{l}{\textbf{Text spec evaluation (pipeline mode)}}\\
\midrule
Avg. LLM-Judge & 0.92 & 0.86 & 0.60 & 0.80 \\
\midrule

\multicolumn{5}{l}{\textbf{Code GT evaluation (code mode)}}\\
\midrule
Avg. LLM-Judge & 0.60 & 0.59 & 0.23 & 0.49 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/general_1.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance of \textsc{DataFlow-Instruct-10K} on Math Benchmarks: Qwen2-7B-Base and Qwen2.5-7B-Base finetuned series of models (Exact Match \%). }
%Blue numbers highlight DF-Gen-10K finetuning, and red numbers highlight the corresponding Instruct checkpoints.
\label{tab:general_math}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} 
& \textbf{MATH} & \textbf{GSM8K} & \textbf{AMC23} & \textbf{AIME24} 
& \textbf{Minerva} & \textbf{Gaokao} & \textbf{Olympiad} & \textbf{Math-Avg} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{9}{c}{\textit{\textbf{Models based on Qwen2-7B}}} \\
\midrule
\textbf{Qwen2-7B-Base}                             & 21.2 & 55.9 & 15.0 & 0.0 &  9.9 & 30.8 &  7.7 & 20.1 \\
\textbf{\quad + Inf-10K}                           & 45.6 & 81.7 & 25.0 & 3.3 & 11.8 & 24.2 & 11.1 & 29.0 \\
\textbf{\quad + Inf-1M}                            & 45.4 & 79.2 & 25.0 & 0.0 & 13.2 & 22.0 & 10.4 & 27.9 \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                        & 54.0 & 83.0 & 27.5 & 0.0 & 16.5 & 25.3 & 20.3 & \textcolor{blue}{32.4} \\
\textbf{Qwen2-7B-Instruct}                         & 53.9 & 86.2 & 22.5 & 3.3 & 17.6 & 35.2 & 19.6 & \textcolor{red}{34.0} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{9}{c}{\textit{\textbf{Models based on Qwen2.5-7B}}} \\
\midrule
\textbf{Qwen2.5-7B-Base}                           & 62.8 & 67.1 & 45.0 & 10.0 & 17.6 & 27.5 & 29.6 & 37.1 \\
\textbf{\quad + Inf-10K}                           & 40.2 & 30.9 & 25.0 & 3.3  &  9.2 & 27.5 & 21.8 & 22.6 \\
\textbf{\quad + Inf-1M}                            & 50.6 & 82.0 & 27.5 & 0.0  & 22.1 & 30.8 & 20.0 & 33.3 \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                        & 73.8 & 88.2 & 47.5 & 16.7 & 30.9 & 31.9 & 37.6 & \textcolor{blue}{46.7} \\
\textbf{Qwen2.5-7B-Instruct}                       & 75.1 & 92.4 & 47.5 & 10.0 & 34.9 & 48.4 & 40.6 & \textcolor{red}{49.8} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/general_2.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance of \textsc{DataFlow-Instruct-10K} on Code and Knowledge benchmarks: Qwen2-7B-Base and Qwen2.5-7B-Base finetuned models.}
\label{tab:general_code_knowledge}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} 
& \textbf{HumanEval} & \textbf{MBPP} & \textbf{Code-Avg} 
& \textbf{MMLU} & \textbf{C-EVAL} & \textbf{Knowledge-Avg} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Models based on Qwen2-7B}}} \\
\midrule
\textbf{Qwen2-7B-Base}                      & 66.5 & 66.1 & 66.3                 & 69.6 & 82.8 & \textcolor{red}{76.2} \\
\textbf{\quad + Inf-10K}                    & 64.0 & 71.7 & 67.8                 & 69.3 & 83.0 & \textcolor{red}{76.2} \\
\textbf{\quad + Inf-1M}                     & 65.9 & 70.4 & \textcolor{blue}{68.2} & 69.5 & 83.0 & \textcolor{red}{76.2} \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                 & 64.6 & 67.7 & 66.2                 & 69.4 & 82.8 & \textcolor{blue}{76.1} \\
\textbf{Qwen2-7B-Instruct}                  & 73.8 & 65.3 & \textcolor{red}{69.6}  & 69.9 & 82.0 & 76.0 \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{7}{c}{\textit{\textbf{Models based on Qwen2.5-7B}}} \\
\midrule
\textbf{Qwen2.5-7B-Base}                    & 78.7 & 74.3 & 76.5                 & 71.9 & 80.0 & \textcolor{blue}{76.0} \\
\textbf{\quad + Inf-10K}                    & 77.4 & 77.8 & 77.6                 & 71.8 & 79.9 & 75.8 \\
\textbf{\quad + Inf-1M}                     & 78.0 & 78.0 & 78.0                 & 72.2 & 79.4 & 75.8 \\
\textbf{\quad + \textsc{DataFlow-Instruct-10K}}                 & 80.5 & 76.7 & \textcolor{blue}{78.6} & 72.1 & 80.2 & \textcolor{red}{76.2} \\
\textbf{Qwen2.5-7B-Instruct}                & 81.7 & 79.4 & \textcolor{red}{80.6}  & 71.8 & 79.6 & 75.7 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/knowledge_cleaning.tex <==
\begin{table}[t]
\centering
\small
\caption{Knowledge Extraction: Accuracy comparison on PubMedQA, Covert, and PubHealth under different reasoning and training settings.}
\label{tab:kbc-result}
\begin{tabular}{lccc}
\toprule
\textbf{Method (ACC)} & \textbf{PubMedQA} & \textbf{Covert} & \textbf{PubHealth} \\
\midrule
\textbf{CoT} & 36.40\% & 48.33\% & 29.00\% \\
\textbf{RAG} & 43.33\% & 17.55\% & 19.60\% \\
\textbf{SFT (DataFlow-Knowledge)} & \textbf{53.40\%} & \textbf{68.33\%} & \textbf{40.86\%} \\
\bottomrule
\end{tabular}

\end{table}


==> tables/reasoning.tex <==
\begin{table}[t]
\centering
\small
\caption{Math Reasoning Pipeline: Performance comparison of Qwen2.5-32B-Instruct under different synthetic data training settings.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\textbf{Model} & \textbf{gsm8k} & \textbf{math} & \textbf{amc23} & \textbf{olympiad} & \textbf{gaokao24\_mix} & \textbf{minerva} & \textbf{AIME24@32} & \textbf{AIME25@32} & \textbf{Avg} \\
\midrule
\textbf{Qwen2.5-32B-Instruct} & 95.8 & 73.5 & 70.0 & 38.5 & 42.9 & 26.5 & 16.8 & 11.6 & 46.95 \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{10}{c}{\textit{\textbf{Trained with 1 epoch}}} \\
\midrule
\textbf{+ SYNTHETIC-1-10k} & 92.9 & 71.8 & 52.5 & 38.4 & 23.1 & 24.3 & 35.6 & 34.0 & 46.6 \\
\textbf{+ Open-R1-10k}     & 91.5 & 72.3 & 65.0 & 38.4 & 20.9 & 24.6 & 43.0 & 33.5 & 48.7 \\
\textbf{+ DataFlow-Reasoning-10K} & 93.9 & 72.3 & 72.5 & 38.7 & 38.5 & 26.5 & 35.9 & 34.5 & \textbf{51.6} \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{10}{c}{\textit{\textbf{Trained with 2 epochs}}} \\
\midrule
\textbf{+ SYNTHETIC-1-10k}  & 94.5 & 78.4 & 75.0 & 45.0 & 24.2 & 28.3 & 48.4 & 37.9 & 54.0 \\
\textbf{+ Open-R1-10k}      & 93.9 & 77.2 & 80.0 & 44.1 & 20.9 & 25.4 & 51.0 & 40.7 & 54.2 \\
\textbf{+ DataFlow-Reasoning-10K} & 94.4 & 76.6 & 75.0 & 45.2 & 42.9 & 25.7 & 45.4 & 40.0 & \textbf{55.7} \\
\bottomrule
\end{tabular}
}
\label{tab:reasoning}
\end{table}


==> tables/text2sql.tex <==
\begin{table*}[t]
\centering
\caption{Text-to-SQL Pipeline: Performance of LLMs on mainstream benchmarks. The first two blocks list closed-source and open-source base models. The last two blocks show fine-tuned models, where the first column indicates the training data setting.}
\label{tab:text2sql_table}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccccccccccccc|cc}
\toprule
\multirow{3}{*}{\textbf{LLM / Training Data}} & \multicolumn{2}{c}{\textbf{Spider}} & \multicolumn{2}{c}{\textbf{Spider}} & \multicolumn{2}{c}{\textbf{BIRD}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{EHRSQL}}} & \multicolumn{2}{c}{\textbf{Spider-}} & \multicolumn{2}{c}{\textbf{Spider-}} & \multicolumn{2}{c|}{\textbf{Spider-}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Average}}}\\

& \multicolumn{2}{c}{\textbf{dev}} & \multicolumn{2}{c}{\textbf{test}} & \multicolumn{2}{c}{\textbf{dev}} & & & \multicolumn{2}{c}{\textbf{DK}}& \multicolumn{2}{c}{\textbf{Syn}} & \multicolumn{2}{c|}{\textbf{Realistic}} & &\\

\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
& Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj & Gre & Maj &Gre & Maj\\

\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Closed-source LLMs}}} \\
\midrule
GPT-4o-mini & 70.4 & 71.0 & 82.4 & 83.7 & 58.8 & 61.5 & 37.9 & 43.1 & 73.3 & 74.4 & 60.5 & 61.6 & 64.4 & 66.7 & 64.0 & 66.0 \\
GPT-4-Turbo & 72.4 & 72.2 & 83.4 & 84.2 & 62.0 & 63.6 & 43.1 & 44.8 & 72.3 & 72.1 & 62.9 & 63.5 & 67.5 & 68.3 & 66.2 & 67.0\\
GPT-4o & 70.9 & 70.7 & 83.2 & 84.9 & 61.9 & 64.0 & 44.9 & 45.5 & 72.9 & 73.5 & 59.6 & 62.3 & 66.5 & 66.7 & 65.7 & 66.8 \\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Open-source LLMs}}} \\
\midrule
DeepSeek-Coder-7B-Instruct & 63.2 & 63.2 & 70.5 & 73.2 & 43.1 & 48.0 & 28.6 & 33.9 & 60.9 & 64.1 & 49.9 & 51.7 & 58.7 & 58.9 & 53.6 & 56.1 \\
Qwen2.5-Coder-7B-Instruct & 73.4 & 77.1 & 82.2 & 85.6 & 50.9 & 61.3 & 24.3 & 36.9 & 67.5 & 73.6 & 63.1 & 66.9 & 66.7 & 70.5 & 61.2 & 67.4\\
Qwen2.5-7B-Instruct & 65.4 & 68.9 & 76.8 & 82.6 & 46.9 & 56.4 & 20.9 & 32.1 & 63.7 & 71.8 & 54.2 & 60.0 & 56.7 & 63.6 & 54.9 & 62.2 \\
OpenCoder-8B-Instruct & 59.5 & 59.5 & 68.3 & 70.1 & 37.5 & 45.3 & 21.9 & 29.9 & 62.6 & 64.7 & 46.0 & 46.1 & 49.0 & 49.4 & 49.3 & 52.1 \\
Meta-Llama-3.1-8B-Instruct & 61.8 & 67.7 & 72.2 & 78.5 & 42.0 & 53.1 & 24.6 & 33.7 & 62.6 & 69.9 & 53.1 & 59.3 & 57.5 & 61.0 & 53.4 & 60.5 \\
Granite-8B-Code-Instruct & 58.5 & 59.2 & 64.9 & 68.6 & 27.6 & 32.5 & 16.0 & 22.6 & 50.7 & 54.4 & 45.0 & 46.8 & 48.8 & 49.4 & 44.5 & 47.6 \\
Granite-3.1-8B-Instruct & 58.3 & 65.0 & 69.8 & 75.3 & 36.0 & 47.2 & 19.6 & 32.3 & 60.0 & 66.5 & 47.7 & 53.8 & 46.5 & 57.1 & 48.3 & 56.7\\
\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Trained on Meta-Llama-3.1-8B-Instruct}}} \\
\midrule
SynSQL(50K) & 67.1 & 73.9 & 72.7 & 78.6 & 49.1 & 55.2 & 33.6 & 40.8 & 63.8 & 66.1 & 59.6 & 63.5 & 69.3 & 71.6 & 59.3 & 64.2 \\

SynSQL(90K) & 68.2 & 74.6 & 73.4 & 78.5 & 51.1 & 54.9 & 31.8 & 38.0 & 61.8 & 67.4 & 58.9 & 63.6 & 69.0 & 70.9 & 59.2 & 64.0 \\

SynSQL(2.5M) & 70.6 & 73.7 & 78.3 & 82.5 & 58.9 & 62.0 & 35.1 & 37.0 & 72.3 & 74.7 & 61.0 & 63.1 & 67.9 & 69.4 & 63.4 & 66.1 \\
\midrule
Spider+BIRD+DataFlow-Text2SQL-90K & 74.9 & 79.2 & 78.4 & 82.3 & 53.4 & 58.9 & 28.4 & 36.5 & 67.7 & 69.7 & 66.6 & 69.1 & 74.4 & 75.0 & 63.4 & 67.2 \\
\midrule
\textbf{DataFlow-Text2SQL-50K} & 69.9 & 76.8 & 75.1 & 80.1 & 51.4 & 57.6 & 28.0 & 36.4 & 65.9 & 68.1 & 61.3 & 67.5 & 69.6 & 73.5 & 60.2 & 65.7 \\
\textbf{DataFlow-Text2SQL-90K} & 71.4 & 76.4 & 75.8 & 80.0 & 54.6 & 56.8 & 55.5 & 56.3 & 66.5 & 67.7 & 61.6 & 67.3 & 71.4 & 72.7 & 65.3 & 68.2 \\


\midrule
\rowcolor[rgb]{.867, .922, .969}
\multicolumn{17}{c}{\textit{\textbf{Trained on Qwen2.5-Coder-7B-Instruct}}} \\
\midrule
SynSQL(50K) & 77.1 & 82.1 & 81.8 & 84.8 & 54.0 & 59.3 & 33.1 & 44.1 & 67.1 & 69.5 & 68.0 & 70.6 & 77.2 & 80.3 & 65.5 & 70.1\\
SynSQL(90K) & 79.2 & 83.1 & 82.3 & 84.4 & 56.2 & 59.4 & 31.4 & 41.4 & 65.0 & 70.7 & 67.2 & 70.7 & 77.0 & 79.9 & 65.5 & 69.9 \\
SynSQL(2.5M) & 81.2 & 81.6 & 87.9 & 88.3 & 63.9 & 66.1 & 34.9 & 40.0 & 76.1 & 77.8 & 69.7 & 69.6 & 76.2 & 78.0 & 70.0 & 71.6 \\
\midrule
Spider+BIRD+DataFlow-Text2SQL-90K & 85.5 & 87.5 & 87.5 & 88.5 & 58.3 & 64.0 & 27.9 & 39.8 & 71.0 & 73.1 & 75.0 & 76.2 & 82.3 & 83.7 & 69.6 & 73.3 \\
\midrule
\textbf{DataFlow-Text2SQL-50K} & 80.9 & 84.9 & 84.6 & 85.8 & 57.9 & 62.5 & 27.8 & 39.4 & 69.7 & 71.2 & 70.0 & 74.0 & 77.8 & 82.1 & 67.0 & 71.4 \\
\textbf{DataFlow-Text2SQL-90K} & 82.0 & 85.0 & 84.8 & 86.0 & 59.2 & 61.5 & 56.1 & 58.7 & 69.7 & 71.0 & 69.9 & 74.4 & 79.5 & 81.7 & 71.6 & 74.0 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/text_conversation.tex <==
\begin{table}[t]
\centering
\small
\caption{Conversation Synthesis: Performance comparison on conversation-domain datasets and general benchmarks for Qwen2.5-7B under different 15K SFT data sources.}
\label{tab:conversation}
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Conversation Benchmarks}} 
& \multicolumn{4}{c}{\textbf{General Benchmarks}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8}
\textbf{Model} 
& \textbf{TopDial} & \textbf{Light} & \textbf{Avg} 
& \textbf{MMLU} & \textbf{AlpacaEval} & \textbf{Arena-Hard} & \textbf{Avg} \\
\midrule
\textbf{Qwen2.5-7B} 
& 7.71 & 7.79 & 7.75 
& 71.45 & 7.05 & 0.60 & 26.36 \\
\textbf{+ ShareGPT-15K} 
& 7.75 & 6.72 & 7.24 
& 73.09 & 3.70 & 1.30 & 26.03 \\
\textbf{+ UltraChat-15K} 
& 7.72 & 6.83 & 7.28 
& 72.97 & 3.97 & 0.80 & 25.91 \\
\textbf{+ DataFlow-Chat-15K} 
& 7.98 & 8.10 & 8.04 
& 73.41 & 10.11 & 1.10 & \textbf{28.21} \\
\bottomrule
\end{tabular}
% }
\end{table}


==> tables/text_pt.tex <==
\begin{table}[t]
\centering
\small
\caption{Pre-training Data Filtering: Performance comparison across models trained with 30B-scale tokens on general evaluation benchmarks.}
% \resizebox{\textwidth}{!}{
\label{tab:PT}
\begin{tabular}{lccccccc}
\toprule
\textbf{Methods} & \textbf{ARC-C} & \textbf{ARC-E} & \textbf{MMLU} & \textbf{HellaSwag} & \textbf{WinoGrande} & \textbf{Gaokao-MathQA} & \textbf{Avg} \\
\midrule
\textbf{Random-30B}      & 25.26 & 43.94 & 27.03 & 37.02 & 50.99 & 27.35 & 35.26 \\
\textbf{Qurating-30B}    & 25.00 & 43.14 & 27.50 & 37.03 & 50.67 & 26.78 & 35.02 \\
\textbf{FineWeb-Edu-30B}  & 26.45 & 45.41 & 27.41 & 38.06 & 50.43 & 25.64 & 35.57 \\
\textbf{DataFlow-30B}    & 25.51 & 45.58 & 27.42 & 37.58 & 50.67 & 27.35 & \textbf{35.69} \\
\bottomrule
\end{tabular}
% }
\end{table}


==> tables/text_sft.tex <==
\begin{table}[t]
\centering
\small
\caption{SFT Data Filtering: Comparison of different 5k dataset filtering methods across Math, Code, and Knowledge benchmarks.}
\label{tab:SFT}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{6}{c}{\textbf{Math}} & \multicolumn{3}{c}{\textbf{Code}} & \multicolumn{3}{c}{\textbf{Knowledge}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\textbf{Methods} & \textbf{math} & \textbf{gsm8k} & \textbf{aime24} & \textbf{minerva} & \textbf{olympiad} & \textbf{Avg} 
& \textbf{HumanEval} & \textbf{MBPP} & \textbf{Avg} 
& \textbf{MMLU} & \textbf{C-EVAL} & \textbf{Avg} \\
\midrule
\textbf{Alpaca(random)} 
& 54.9 & 77.2 & 13.3 & 14.0 & 27.0 & 37.3 
& 71.3 & 75.9 & 73.6 
& 71.8 & 80.0 & 75.9 \\
\textbf{Alpaca(filtered)} 
& 60.3 & 80.0 & 13.3 & 14.7 & 30.7 & 39.8 
& 73.8 & 75.7 & 74.8 
& 71.8 & 80.0 & 75.9 \\
\midrule
\textbf{WizardLM(random)} 
& 61.1 & 84.2 & 6.7 & 18.0 & 29.3 & 39.9 
& 75.6 & 82.0 & \textbf{78.8} 
& 71.8 & 79.2 & 75.5 \\
\textbf{WizardLM(filtered)} 
& 69.7 & 88.8 & 10.0 & 19.9 & 35.4 & 44.8 
& 77.4 & 80.4 & \textbf{78.9} 
& 71.9 & 79.6 & 75.8 \\
\midrule
\textbf{DataFlow-SFT-15K(random)} 
& 72.6 & 89.6 & 13.3 & 37.9 & 32.9 & \textbf{49.3} 
& 79.9 & 75.9 & 77.9 
& 72.1 & 80.0 & \textbf{76.1} \\
\textbf{DataFlow-SFT-15K(filtered)} 
& 73.3 & 90.2 & 13.3 & 36.0 & 35.9 & \textbf{49.7} 
& 82.9 & 74.9 & \textbf{78.9} 
& 72.2 & 80.4 & \textbf{76.3} \\
\bottomrule
\end{tabular}
}
\end{table}

